Latency-Aware Inter-domain Routing

Despite efforts from cloud and content providers to lower latency to acceptable levels for current and future services (e.g., augmented reality or cloud gaming), there are still opportunities for improvement. A major reason that traffic engineering efforts are challenged to lower latency is that the Internet's inter-domain routing protocol, the Border Gateway Protocol, is oblivious to any performance metric, and circuitous routing is still pervasive. In this work, we propose two implementation modifications that networks can leverage to make BGP latency-aware and reduce excessive latency inflation. These proposals, latency-proportional AS prepending and local preference neutralization, show promise towards providing a method for propagating abstract latency information with a reasonable increase in routing overhead.

==> cutoff/intro.tex <==
\section{Introduction}

% Problem

% "We also found that inter-domain routing causes significant path inflation, with almost half the paths being inflated, not because of policies arising out of commercial concerns, but because shortest AS path is the default.'' From causes of path inflation

The Border Gateway Protocol (BGP)~\cite{rfc4271_bgp} is known to
sometimes find excessively long
routes. In~\cite{SIGCOMM03-PathInflation}, Spring et al.  showned
that ``inter-domain routing causes significant path inflation''
despite ISPs' willingness to find shorter paths for their
customers. Researchers have also shown that IP anycast systems may
experience anycast path inflation, where clients are routed to anycast
replicas continents away, due to BGP's poor path choices~\cite{Li2018Internet,beatbgp-todd-hotnet18}.
Even cloud providers with their private wide area networks (WANs) are
not spared of BGP sub-optimality. In ~\cite{INFOCOM20-PrivateWAN}, Arnold et al. showed
that BGP often failed to find paths with the lowest latency for cloud
traffic.

A direct consequence of path inflation is latency inflation.
End-to-end round trip times (RTTs) can be inflated by tens of
milliseconds if packets were detoured by a continent. Yet many
Internet applications -- such as cloud gaming, web, video
conferencing, and online streaming -- demand low latency~\cite{hotnets-edge-computing}.

% Why is it hard?

BGP's path inflation problem has been observed for more than two
decades~\cite{SIGCOMM03-PathInflation,Li2018Internet}. Yet the reality has not changed much. With the
advancement of software defined networking (SDN)~\cite{rizvi2022anycast}, large
providers can alleviate this problem to some extent by using
SDN-WAN~\cite{schlinker2017edge,espresso} to override BGP choices for
their outbound traffic, but the inbound traffic may continue to
experience path inflation.  Similarly, overlay routing can overcome
BGP routing inefficiencies to some extent~\cite{Chen2015End, detour}, but
it requires the deployment of new overlay infrastructure.

% In addition, because there are simply too
% many IP prefixes, BGP overriding may not be universal. As we will show
% in \S~\ref{xxx}, in a recent measurement study, we find that large
% cloud providers still experience path inflation with 100+ ms
% addititive latencies.

% For instance, in the case of IP anycast, xxxx cite the figure.

What adds more to the challenges is that not all BGP paths are bad. In
fact, as articulated in~\cite{beatbgp-todd-hotnet18}, BGP
finds low latency and high throughput paths for the majority of times.
Because BGP is good most of the times, and it is battle-tested,
replacing it with a brand-new inter-domain routing
protocol~\cite{Li2018Internet,rfc7311_abgp} is utterly undesirable.


% Yet the status quo is unsatisfactory neither. First of all, routing is
% all about finding paths. When there exists a shorter path, not being
% able to find it and use it is intellectually unsavory to some. Second,
% latencies affect user experiences and hence online sales~\cite{xxx}.

% How did we solve it?

% to make BGP find low-latency paths wherever it matters.
% Because a provider can use traffic engineering techniques to
% steer their outbound traffic to low-latency paths, we focus on
% addressing the inbound traffic path inflation problem in this
% work. 

In this paper, we ask this question: can we address the BGP path
inflation problem without replacing it?  We postulate that in certain
use cases, such as IP anycast, where anycast providers employ replicas
to bring content closer to users, and cloud routing, whereas providers
build out private WANs to satisfy the qualtiy of service requirements
of their customers, low-latency routing is highly desirable.

To this end, we propose a few modifications to the current BGP's
deployment to enable latency-aware BGP routing. Our proposed
modifications use AS path prepending to encode the path length between
two BGP speakers so that shorter AS paths lead to shorter network
distances. In addition, we propose that an IP anycast or a cloud
provider designate specific IP prefixes to carry latency-sensitive
traffic, and negotiate business relatinoships to cover the transit
costs to traffic associated with these IP prefixes. With this business
agreement, other ISPs have incentives to obviate the common
prefer-customer or prefer-peer BGP policies and choose the BGP routes
based on AS path lengths to reach those latency-sensitive IP
prefixes. These modifications together address the root causes of
BGP's latency-oblivious routing problem~\ref{sec:} and do not require
significant modifications to BGP.

% TODO

To gain insights into how well the proposed techniques work, we use a
router-level Internet-topology provided by CAIDA to simulate the above
BGP modifications, and compare the latency improvement results with an
optimal routing protocol that uses latency as the routing metric for
route selection. Our simulation results show that compared to vanilla
BGP, our proposed latency-aware BGP modifications reduce the 80\%
end-to-end latency by xx\% and incur half of the message overhead
compared to the optimal latency-based routing protocol.

% run simulations and show they effectively
% provide low latency routing. We compare with two alternative
% proposals, acumulated IGP~\cite{xxx}, and adding geohints to BGP
% announcements~\cite{xxx}, and show they achieve a better tradeoff
% between convergence and latency than the two alternatives



==> cutoff/method.tex <==
\section{Latency-Aware BGP}
\begin{figure}[t]
    \includegraphics[width=0.9\columnwidth]{figures/as_prepend.pdf}
    \caption{An example of prepending AS number to encode the latency information in BGP. The arrows refer to messages' direction.\label{fig:as_prepend}}
\end{figure}

% In this section, we propose simple modifications to how BGP is deployed to make it latency-aware. We first describe the rationale behind our proposal, then the modifications, and finally the pros and cons of the proposal.
%

These examples, and others discussed in prior work on anycast~\cite{zhihao, us,heiderman-pam} highlight two causes of BGP path inflation: BGP is latency-oblivious, and its policy preferences may lead BGP to select higher latency paths.

The examples we present in the previous section and various examples
presented by previous work in IP anycast studies highlight two primary causes of path inflation in
BGP. First, BGP lacks a latency-related path selection
metric. Hence, it is latency oblivious. Second, local preference
settings may lead BGP to favor routes that do not offer the best
performance. Therefore, the logical steps to enable BGP latency-aware
are to address these two root causes.

\subsection{Latency-Based AS Prepending}

In theory, if we introduce an accumulated latency attribute in BGP,
for instance, a metric similar to the accumualted IGP metric
(AIGP)~\cite{RFC7311-AIGP}, we can enable latency-aware path selection
in BGP. However, such an approach faces deployment and scalability
challenges at the Internet scale. A new BGP attribute requires
modifications to BGP implementations. Additionally, each router-level
path on the Internet is likely to have a different latency
value. Therefore, this metric will expose an AS's router-level details
to other ASes, leading to inter-domain path implosion.

These challenges prompt us to explore alternative methods to embed
latency information within existing BGP attributes. Notably, one of
the high-order BGP tie breakers is the AS path length. However, this
attribute lacks meaningful semantics because AS sizes differ
significantly.  This realization leads us to consider using AS
prepending for embedding latency information in BGP.

Specifically, if when a path traverses a large AS, the large AS
prepends itself multiple times in the BGP AS path attribute, then the
AS path length in a BGP route advertisement would align closely
with the actual path length. Since path length
correlates with network propagation latency, and BGP already uses AS
path length as tie-breakers in its path selection algorithm, this AS
prepending method can effectively introduce latency awareness into BGP.

% In this paper, we propose a mechanism to enable BGP's awareness of latency by encoding the path latency with AS prepending. The key idea is that an AS prepend its ASN one or more times according to the latency estimation it needs to transit the packet.

We use Figure~\ref{fig:as_prepend} to explain the idea. In the
figure, $AS1$ and $AS2$ have an exterior BGP (eBGP) session between
their border routers $R2$ and $R3$. Routers $R1$ and $R2$ in $AS1$
have an interior BGP (iBGP) session. Suppose the
router $R1$ propagates a route advertisement of an IP prefix to
router $R2$, which in turn exports it to its eBGP neighbor $R3$.

In the current BGP, $R2$ will prepend its AS number ($AS1$) in the AS
path attribute of the BGP advertisement when it exports the route to
$R3$. With our proposed modification, $R2$ will prepend its AS number
multiple times according to the propagation latency 
between itself and its eBGP neighbor
$R3$.
We propose to use the minimum propagation latency that is determined by the underlying network infrastructure and the speed-of-light constraint to ensure routing stability.
The exact number of times $R2$ prepends its AS numbers is computed by normalizing the minimum propagation latency with a quantization factor $Q$:
$\Bigl\lfloor \frac{L(R2,R3)}{Q} \Bigr\rfloor+1$,
where $L(R2,R3)$ denotes the latency between $R2$ and $R3$, 
and $\lfloor x \rfloor$ denotes the floor integer value of a real number $x$. For eBGP sessions, the minimum number of AS prepending is one, consistent with the current BGP specification. 

For an iBGP session, we propose to use a receiver-prepending mechanism.
That is, when $R2$ receives the route from $R1$, it prepends its AS
number according to the minimum propagation latency between itself and
$R1$: $\Bigl\lfloor \frac{L(R1,R2)}{Q} \Bigr\rfloor$.  
Because an AS may employ route reflectors~\cite{RFC4456-RouteReflection}, 
the first border router in an iBGP session (\eg, $R1$) may
not know the other border router that will receive its route
advertisement (\eg, $R2$).  A receiver-prepending mechanism addresses
this nuance. $R2$ can use the next hop attribute to determine the 
minimum propagation latency between $R1$ and $R2$, 
as the method used by AIGP~\cite{RFC7311-AIGP}.
%as an iBGP route propagated by $R1$ will have its IP
%address in the next hop attribute, and $R2$ can use this field to
%determine the static propagation latency between $R1$ and $R2$ and
% prepends the AS path length accordingly. 

% As shown by the formulas, we prepend AS at least once in an eBGP
% session to avoid AS loop during propagation, but we may not prepend AS
% in an iBGP session to avoid unnecessary prepending if the latency
% between two routers are small than $Q$ (\eg, $R1$ and $R2$).

Because in most scenarios BGP can select a good
path~\cite{beatbgp-todd-hotnet18}, we can tune the quantization factor $Q$
to balance the number of different AS path
lengths an AS exports to its neighbors and latency optimization. In
\S~\ref{sec:simulation}, we use simulations to show how the
quantization factor affects routing overhead and performance. % future work

Embedding latency information using AS prepending offers several
advantages. Firstly, it avoid introducing new attributes to BGP, as
BGP already supports AS path and AS prepending.  Besides, an ISP only
needs to enable this AS prepending method for specific
latency-sensitive prefixes without universal deployments, as BGP
route selection is per-prefix based
% and ASes can agree upon certain IP prefixes as latency-sensitive, and change their AS prepending configurations for those prefixes.
Second, because of the introduction of the quantization factor, this method is coarse-grained. Therefore, it does not expose significant details of an AS's internal topology or routing policies, alleviating privacy concerns.
In addition, it can  avoid overly circuitous paths while offering sufficient choices of equal-length AS paths for traffic engineering. 
Finally, due to the coarse-grained nature of AS prepending, it shows the potential to scale to the size of the Internet without excessively increasing the number of advertisements used for BGP convergence, as we will present in \S~\ref{sec:simulation}.

\subsection{Local Preference Neutralization}

% When examining the cases presented in \S~\ref{sec:example}, we notice that
% latency-aware AS prepending allows BGP to select the better
% router in Case~1, as in both cases, the better route shares
% the same local preference as the other less optimal route according to  common BGP
% policies. However, it proves ineffective in Case~2, where the less-optimal
% route, the peer route, is preferred over the better provider router.

A second main cause to BGP path inflation is policy routing. To fix this problem, we need to neutralize BGP's local preferences.
This is generally infeasible, as local preferences are commonly set to maximize an ISP's profit.
However, since local preference settings are driven by commerical interests, we speculate that in certain scenarios where the finanical benefit gained from delivering content in a low-latency manner significantly offsets the network transit costs, a cloud or a content provider will be willing to cover the transit costs for its own traffic end-to-end.
When such finanical incentives exist, a cloud provider or an IP anycast CDN can elect specific IP prefixes to carry latency-sensitive traffic, and negotiate business agreements with its neighboring ASes to cover both the ``up-hill'' and the ``down-hill'' transit costs~\cite{gao-} associated with those IP prefixes.
With this financial agreement, the cloud's or the CDN's neighboring ASes and their customers need not worry about the transit costs for these latency-sensitive IP prefixes. Thus, they can set the local preferences to these IP prefixes to the same value and select a path to these IP prefixes based on the latency-base AS path length.

For the outbound traffic from these latency-sensitive IP prefixes, a cloud provider or an IP anycast CDN can neutralize the local preferences to routes learned from all its neighbors, enabling route selection based on the latency-aware AS path length.

Local preference neutralization does not violate BGP's valley-free
routing policy, which is essential to guarantee that BGP
converges~\cite{ToN01-GaoRexford,ToN01-ASRel}. The reason is that
valley-free routing is governed by BGP's route export policies,
whereas local preferences are set by BGP's import policies. As long as
BGP routers continue to follow the valley-free route export policies,
such as only exporting provider or peer routes to customers, they will
continue to select valley-free routes.

% At first glance, convincing other ASes to neutralize their local
% preferences for certain routes seems daunting. However, given the
% increasingly flat structure of the Internet~\cite{xxx} and the fact
% that most routing inefficiencies occur between large providers, we
% speculate that if a cloud provider or a CDN can persuade the large
% ASes it peer with or its transit providers to inform their customers
% to neutralize their local preferences, many routing inefficiencices
% could be mitigated.
% 

In cases where neutralizing local preferences is not feasible, we hypothesize that latency-based AS prepending alone can still mitigate path inflation to certain extent. This is supported by a previous study that shows most path inflation arises from using the shortest AS path metric for BGP path selection, while policies such as valley-free or prefer-customer are not a significant contributor~\cite{SIGCOMM03-PathInflation}. However, given that the study was conducted two decades ago, and the Internet has since become much flatter, we are uncertain if this conclusion still holds. It is our future work to validate this hypothesis.


% $AS1$ and $AS2$ may have any relationship (peer-to-peer,
% provider-to-customer, or customer-to-provider). $AS1$ intends to
% announce a BGP route for a prefix $P$ to $AS2$. In $AS1$, the BGP
% advertisement comes from $R1$, which may either be the origin of the
% prefix or may received the advertisement from another AS via an
% exterior BGP (eBGP) session. $R1$ uses an interior BGP (iBGP) session
% to announce the route advertisement to $R2$ without adding ASN to the AS path field. When $R2$ to propagates to $R3$ by EBGP, $R2$ generates a BGP update message by appending $AS2$ to the AS path by a number of times according to the following formula:
% 
% In the formula, $L(A,B)$ refers to the latency between routers $A$ and $B$, which can be estimated by the half of the RTT between them. $Q$ is an quantization factor, which quantize the latency to the number of appending times. $Q$ is necessary because the latency between two endpoints can be dynamic, and we use to $Q$ to eliminate the small fluctuation of latency to avoid unnecessary BGP updates. $\lceil x \rceil$ means the ceiling integer of a real number $x$. Overall, the formula calculates the interior latency and exterior to transit a packet and quantize it to a integer representing the number of AS appending times.
% For example, suppose the latency between $R1$ and $R2$ is 110~ms and the latency between $R2$ and $R3$ is 20~ms. When $AS1$ takes $Q=50~ms$, meaning that it does not care about the latency difference less than $50~ms$. Thus, according to the formula, $R2$ will append $\lceil \frac{110+20}{50} \rceil=3$ times of $AS1$ to the AS path field in the EBGP message announced to $R3$.
% 
% Besides, an AS may propagate the BGP update to different ASes, or it may propagate to one AS through different routers. This causes BGP path diversity and different paths may holds different latency. The AS can configure its routers to generate EBGP messages with different AS appending counts for those paths. For consistency, An AS should uses the same $Q$ for each message. When an AS receives multiple BGP updates for the same prefix, it naturally prefer the path with shorter AS path length, which indicating a path with a lower latency.
% Therefore, such a simple mechanism enables BGP to be aware of path latency.
% 
% We note that the proposed mechanism is similar to AIGP, which embedded the IGP cost into BGP and accumulated the IGP cost over the AS path. However, AIGP requires an additional field in BGP, and the AS receiving the BGP update should be enable to recognize the field during the path selection. Because of the decentralization feature of the Internet, it is hard for an AS which intends to adopt AIGP to persuade the other ASes to also adopt AIGP. In contrast, our mechanism avoid such tedious upgrade for multiple ASes, because we encode the latency information into the existing AS path field. Not only the ASes around the world can recognize this field but also they already considered preferring shorter AS path in their BGP best path selection algorithms.
% 

\subsection{Put it Together}

discuss how the methods proposed can fix the examples.


==> cutoff/motivation.tex <==
\section{BGP Path Inflation}
\label{sec:motivation}

In this section, we first summarize BGP's best path selection
algorithm. We then use two concrete examples to analyze the root
causes of BGP path inflation.

\subsection{BGP Best Path Selection Algorithm}\label{sec:bgp_select}

% It was designed as a policy routing protocol that facilitates business
% relationships between ISPs.

Unlike intra-domain routing protocols~\cite{ospf,is-is}, BGP does not use a single optimization metric for route selection. Each BGP route is associated with a tuple of attributes, and the BGP best path selection is based on the ordered comparison of the attributes of two routes.

According to BGP's specification~\cite{rfc4271_bgp}, the most significant
attribute in its route selection process is the local preference, which is
set according to a BGP router's local policy. For routes to the same
destination with the same local preference, a BGP speaker then uses a
tie-breaking algorithm that compares AS path lengths, route origins,
the multi-exit descriminators, an eBGP or iBGP path, interior routing
costs, and other parameters until the best route is selected.

In practice, the local preferences are set according to business
relatinoships between ISPs. Routes advertised by customers are
preferred over those advertised by peers (prefer-customer), and routes
advertised by peers are preferred over those advertised by transit
providers (prefer-peer).

\subsection{Examples of Path Inflation in BGP}\label{sec:example}

Historically, infrastructure and routing policy are the two main
factors that contribute to path inflation on the
Internet~\cite{SIGCOMM03-PathInflation}. While infrastructure
investment such as more direct paths~\cite{NSDI22-cisp} and broad
peering can reduce path inflation, hence latency inflation, we use
concrete examples from real-world network traces to illustrate that
given the existing infrastructure, BGP's path selection process still
has significant impacts on end-to-end path inflation. In the examples
we show, shorter and valley-free paths~\cite{gaoRexford} exist. Yet
BGP fails to find those paths.

\begin{figure}[h]
    \centering
    \begin{minipage}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eg_angola.png}
        %\caption{\azure}
    \end{minipage}% 
    \caption{A RIPE Atlas probe located in Fortaleza, Brazil takes the solid line path to reach the Internet-transit IP address of an Azure VM located in Johannesburg, South Africa. In contrast, the same probe reaches the same VM's private WAN-transit IP address via the dotted line path. Colors encode path segments in different ASes.\label{fig:case1}}
\end{figure}

\begin{figure}[h]
    \centering
    % \begin{minipage}[b]{0.48\textwidth}
    %     \centering
    %     \subcaptionbox{Part of Angola Cables' network map~\cite{AngolaMap}\label{fig:cable:angola}}{\includegraphics[width=\linewidth]{figures/angola_cable.png}}
    % \end{minipage}% 
    \begin{minipage}[b]{0.48\textwidth}
        \centering
        \subcaptionbox{Part of Azure's network map~\cite{MicrosoftMap}\label{fig:cable:azure}}{\includegraphics[width=\linewidth]{figures/azure_cable_with_sacs.png}}
    \end{minipage}% 
    \caption{Part of network infrastructure map of (a) Angola Cables and (b) Azure.\label{fig:network_map}}
\end{figure}

\paragraph{Case 1:} In the first example, the cloud provider Azure
peers with the ISP Angola Cables at two places S\~{a}o Paulo, Brazil
and Johannesburg, South Africa. Azure also has a datacenter in
Johannesburg~\cite{azure-pops} and owns a private WAN. It offers
two types of transit services~\cite{azure} for its customers'
virtual machines (VMs): one service transits via its private WAN as
much as possible and the other uses the public Internet for transit
service. If a VM located at Azure's Johannesburg datacenter chooses to
use the private WAN transit service, Azure will advertise its IP
prefix at both Johannesburg and S\~{a}o Paulo. In contrast, if a VM
chooses to to use the public Internet for transit service, Azure will
only advertise its IP prefix in the Johannesburg region.

When we send packets from a RIPE Altas probe~\cite{candela-RIPEloc-19Access} probe
located in Fortaleza, Brazil (probe ID: 50734) to the private-WAN
transit IP address of a VM, we obtain a 254~ms round trip time
(RTT). In contrast, the RTT from the same probe to the same VM
with the Internet transit IP address has an RTT of 115~ms.

What have caused this large RTT discrepancy between the same pair of
endpoints?  By examining the traceroutes and network topologies of
Angola Cables~\cite{AngolaMap} (Figure~\ref{fig:cable:angola}) and
Azure~\cite{MicrosoftMap} (Figure~\ref{fig:azure}), we find that the
latency difference comes from the fact that Azure does not own direct
submarine cables between South America and Africa, while Angola Cables
owns one. When a VM's Internet-transit IP prefix is only advertised in
Johannesburg, Angola Cables uses its own submarine cable to deliver
the probe's traffic through the South Atlantic Ocean to South Africa,
and the traffic enters Azure in Johannesburg, as shown by the solid
line path in Figure~\ref{fig:case1}. In contrast, when a VM's privat
WAN-transit IP prefix is advertised at both both S\~{a}o Paulo and
Johannesburg, Angola Cables sends the probe's traffic to S\~{a}o
Paulo, resulting in the much longer dotted-line path shown in
Figure~\ref{fig:case1}.

% However, in the private WAN transit service, because Azure announces
% the IP prefix also at S\~{a}o Paulo, the ISP Angola Cables can choose
% between the routes advertised at these two locations.  

Given that the private-WAN IP prefix is advertised at both S\~{a}o
Paulo and Johannesburg, why does BGP fail to choose the shorter path?
We analyze BGP's best route selection algorithm for answers.
According to the algorithm, the route advertised at S\~{a}o Paulo and
Johannesburg likely share the same local preferences, as  the peering AS at both
locations is  Azure. Similarly, the AS path
lengths of the two routes are identical. BGP's tie-breaking algorithm
then relies on  the interior routing costs to break the tie. In this case,
the S\~{a}o Paulo peering location between Azure and Angola Cables is
much closer to the probe than the Johannesburg's peering
location. Consequently, the traffic will take exit  Angola
Cables early at S\~{a}o Paulo, leading to a much more circuitous path.

% by the PoPs around the world, Angola Cable delivers the packet to
% Azure very early through the PoP in S\~{a}o Paulo, Brazil. Since Azure
% does not own a submarine cable in South Atlantic Ocean, it carries the
% packet to the North America and Europe, and then finally reaches the
% Africa, which leads to a significant detour and latency
% inflation. Besides, Azure will not ask for the other ISP to transit
% the packet after it obtains the packet in S\~{a}o Paulo, since the
% destination is within Azure network.
% 

% Figure~\ref{fig:angola} shows an example of inflation caused by BGP's unawareness of network topology. In this example, an vantage point of Angola Cables (AS~37468) in Fortaleza, Brazil sends ping requests to a VM of Azure (AS~8075) in Johannesburg, South Africa through \wan and \inet services, respectively.
% Surprisingly, it takes 254~ms for \wan service but 115~ms for \inet service, which is contrary to the intuition that \wan service should provide lower latency.

% In this case, BGP fails to find the path with shorter-latency between
% the route advertised at S\~{a}o Paulo and the one advertised at
% Johannesburg because there is no metric in its best path selection
% algorithm that informs BGP of the path latency.

\begin{figure}[h]
    \centering
    \begin{minipage}[b]{0.40\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eg_google.png}
        %\caption{\azure}
    \end{minipage}% 
    \caption{A RIPE Atlas probe located at Perth, Australia takes the dotted line path to reach the private-WAN transit IP address of a Google VM located in Mumbai, India. The same probe takes the solid line path to reach the Internet transit IP address of the same VM. Colors encode path segments inside different ASes. \label{fig:case2}}
\end{figure}

\paragraph{Case 2:} In the second case,  we send ping packets from a
RIPE Atlas probe (probe ID: 17003) located in Perth, Australia, to the
IP address of a private-WAN transit VM in Google's Mumbai, India,
datacenter. The RTT of this path is 196~ms. However, a shorter and
valley-free path, with a RTT of 149~ms, exists between the probe and
Google's Mumbai datacenter, as validated by the ping latency from the
probe to the VM's Internet transit IP address. From the traceroute
outputs, we find that the path to the private-WAN transit IP address
enters Google's WAN at Sydney, where the probe's ISP (AARNet) and
Google peer, as shown by the dotted line in Figure~\ref{fig:case2}.
Differently, for the Internet-transit traffic,  the probe's ISP
sends the probe's traffic to Singapore, where it enters the NTT
network and then TATA, which transits the traffic from Singapore to
Mumbai, as shown by the solid line in Figure~\ref{fig:case2}.

In this case, the BGP router at the probe's local ISP AARNet fails to
find the shorter path that exits its network in Singapore. \xy{In
  fact, Google peers with TATA's network in Singapore~\cite{xx} and
  the probe traffic could have entered Google in Singapore.}  We
speculate the reason is the prefer-peer routing policy: Google's route
is a peer route to AARNet, while NTT's route is a provider route,
since NTT is a tier-1 ISP. Another possible explanation is that AARNet
prefers a shorter AS path to reach Google than the longer path that
traverses NTT and TATA.

% the perfer-peer-to-provider routing policy. The
% probe's ISP prefers the peering connection with Google at Syndey to
% the transit connection with NTT at Singapore, leading to an inflated
% latency of more than xx~ms.

% We show another example in Figure~\ref{fig:russia}. The vantage point belongs to Rostelecom (AS~12389) and is located in Vladivostok, Russia, a city in east Asia and near Japan, and the destination is a Azure VM in Frankfurt, Germany. \wan service shows a latency of 222~ms, while \inet service only takes 145~ms. The root cause also lies in the infrastructure difference. In \inet service, Rostelecom carries the packet from the east coast of Russia to Europe by traversing the whole Russia~\cite{RostelecomMap}. It uses Arelion (Twelve99, AS~1299) as the transit provider in Stockholm, Sweden and Arelion deliver the packet to Azure through the PoP in Frankfurt. In contrast, for \wan service, Rostelecom delivers the packet to a Azure's PoP in Tokyo, Japan which is very close to the vantage point. Since Azure has no cable crossing Asia, the packet detours to Singapore and Indian Ocean and then reaches Europe, leading to much higher latency.


\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{0.9\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eg_anycast.png}
    \end{minipage}% 
    \caption{Routes of Case 3\label{fig:case3}}
\end{figure*}

\paragraph{Case 3:} Finally, we show an example observed in the
context of IP anycast~\cite{SIGCOMM23-RegionalCDN}\zx{I put a brand new example here}.
In this case, a CDN
provider Imperva has a site located in Singapore and a site located in
\zx{Amsterdam}, NE. Imperva uses global IP anycast for its DNS service,
and regional IP anycast for its CDN service. Its regional IP anycast
CDN advertises different regional IP anycast prefixes in the Singapore
site and in the \zx{Amsterdam} site, while its global IP anyast DNS service
advertises one global IP anycast prefix at both sites.

A RIPE Atlas probe \zx{(probe ID:1003747)} located in \zx{Rotterdam, NE} reaches
Imperva's global anycast address at the Singapore site, resulting in a
300+~ms RTT. In contrast, the same probe reaches the regional anycast
address at the \zx{Amsterdam} site, with a \zx{13}~ms RTT.

The probe fails to reach the \zx{Amsterdam} site in the global anycast case
for a reason similar to why the probe takes a longer path to reach the
Google private-WAN transit VM in Mumbai. From the traceroute outputs,
we observe that the probe's transit provider is TATA. Imperva's
Singapore site uses SingTel as its transit provider, while its \zx{Amsterdam}
site uses Level3 as its transit provider. SingTel is TATA's customer,
while Level3 is TATA's peer. Because of the prefer-customer routing
policy, TATA prefers the route advertised by SingTel to the route
advertised by Level3 to reach the same global IP anycast prefix.



% These solutions fall into two broad categories of solutions. The first
% category of solutions propose new routing architectures~\cite{xxx} to
% replace BGP~\cite{xxxx}, while the second category of solutions aim to
% enhance BGP with latency-related information~\cite{xxx}. While new
% routing architectures are intellectually stimulating and beneficial in
% the long term, we focus our discussion on BGP-compatible solutions.

% algorithm or architecture for a system construct
% a new system construct



